Management of Electric Vehicles as Flexibility Resource for Optimized Integration of Renewable Energy with Large Buildings

The increasing penetration of renewable generation requires new tools to achieve a high matching between demand and renewable generation at building and community levels. Large commercial and public buildings with parking lots have a considerable potential to provide energy flexibility by controlling the charging of Electric Vehicles (EVs) and injecting part of the stored energy into the building, using Building-to-Vehicle (B2V) and Vehicle-to-Building (V2B) systems. However, EVs and buildings do not often belong to the same entity and in Portugal the existing regulation does not allow financial transactions between buildings and EVs as separate entities. Addressing this regulation hurdle requires innovative optimization methods for the implementation of B2V/V2B systems. Moreover, the new legislation regarding the self-consumption of renewable generation in Portugal enables the trade of renewable generation surplus between buildings and the establishment of renewable energy communities. This paper intends to address this issue and proposes a formulation to aggregate and manage the sharing of generation surplus between buildings, using EVs as a flexibility resource. The simulation results showcase the achieved increase in renewable self-consumption at building and community levels, as well as the reduction in electricity costs.

==> bibliography/output.tex <==
% Generated by IEEEtran.bst, version: 1.12 (2007/01/11)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Delgado2018}
\BIBentryALTinterwordspacing
J.~Delgado, R.~Faria, P.~Moura, and A.~de~Almeida, ``Impacts of plug-in
  electric vehicles in the portuguese electrical grid,'' \emph{Transportation
  Research Part D: Transport and Environment}, vol.~62, pp. 372 -- 385, 2018.
  [Online]. Available: \url{https://doi.org/10.1016/j.trd.2018.03.005}
\BIBentrySTDinterwordspacing

\bibitem{RNC2050}
Portugal, ``Roadmap for carbon neutrality 2050,'' Portuguese Republic, Tech.
  Rep., 2019.

\bibitem{moura2020linking}
P.~Moura, G.~Yu, S.~Sarkar, and J.~Mohammadi, ``Linking parking and electricity
  values to unlock potentials of electric vehicles in portuguese buildings,''
  in \emph{PES General Meeting}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE,
  2020.

\bibitem{Gray2018}
\BIBentryALTinterwordspacing
M.~K. {Gray} and W.~G. {Morsi}, ``A novel transactive energy framework for
  prosumers with battery storage and electric vehicles,'' in \emph{2018 IEEE
  Electrical Power and Energy Conference (EPEC)}, Oct 2018, pp. 1--6. [Online].
  Available: \url{https://doi.org/10.1109/EPEC.2018.8598368}
\BIBentrySTDinterwordspacing

\bibitem{Liu2019b}
\BIBentryALTinterwordspacing
Z.~{Liu}, Q.~{Wu}, K.~{Ma}, M.~{Shahidehpour}, Y.~{Xue}, and S.~{Huang},
  ``Two-stage optimal scheduling of electric vehicle charging based on
  transactive control,'' \emph{IEEE Transactions on Smart Grid}, vol.~10,
  no.~3, pp. 2948--2958, May 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TSG.2018.2815593}
\BIBentrySTDinterwordspacing

\bibitem{Jin2017}
\BIBentryALTinterwordspacing
X.~Jin, J.~Wu, Y.~Mu, M.~Wang, X.~Xu, and H.~Jia, ``Hierarchical microgrid
  energy management in an office building,'' \emph{Applied Energy}, vol. 208,
  pp. 480 -- 494, 2017. [Online]. Available:
  \url{https://doi.org/10.1016/j.apenergy.2017.10.002}
\BIBentrySTDinterwordspacing

\bibitem{Thomas2018}
\BIBentryALTinterwordspacing
D.~Thomas, O.~Deblecker, and C.~S. Ioakimidis, ``Optimal operation of an energy
  management system for a grid-connected smart building considering
  photovoltaics’ uncertainty and stochastic electric vehicles’ driving
  schedule,'' \emph{Applied Energy}, vol. 210, pp. 1188 -- 1206, 2018.
  [Online]. Available: \url{https://doi.org/10.1016/j.apenergy.2017.07.035}
\BIBentrySTDinterwordspacing

\bibitem{Nefedov2018}
\BIBentryALTinterwordspacing
E.~Nefedov, S.~Sierla, and V.~Vyatkin, ``Internet of energy approach for
  sustainable use of electric vehicles as energy storage of prosumer
  buildings,'' \emph{Energies}, vol.~11, no.~8, 2018. [Online]. Available:
  \url{https://doi.org/10.3390/en11082165}
\BIBentrySTDinterwordspacing

\bibitem{Quddus2018}
\BIBentryALTinterwordspacing
M.~A. Quddus, O.~Shahvari, M.~Marufuzzaman, J.~M. Usher, and R.~Jaradat, ``A
  collaborative energy sharing optimization model among electric vehicle
  charging stations, commercial buildings, and power grid,'' \emph{Applied
  Energy}, vol. 229, pp. 841 -- 857, 2018. [Online]. Available:
  \url{https://doi.org/10.1016/j.apenergy.2018.08.018}
\BIBentrySTDinterwordspacing

\bibitem{Liu2019}
\BIBentryALTinterwordspacing
Z.~{Liu}, Q.~{Wu}, M.~{Shahidehpour}, C.~{Li}, S.~{Huang}, and W.~{Wei},
  ``Transactive real-time electric vehicle charging management for commercial
  buildings with pv on-site generation,'' \emph{IEEE Transactions on Smart
  Grid}, vol.~10, no.~5, pp. 4939--4950, Sep. 2019. [Online]. Available:
  \url{https://doi.org/10.1109/TSG.2018.2871171}
\BIBentrySTDinterwordspacing

\bibitem{Fonseca2018}
\BIBentryALTinterwordspacing
P.~{Fonseca}, P.~{Moura}, H.~{Jorge}, and A.~T. {de Almeida}, ``Sustainability
  in university campus: options for achieving nearly zero energy goals,''
  vol.~19, no.~4, pp. 790--816, Jan. [Online]. Available:
  \url{https://doi.org/10.1108/IJSHE-09-2017-0145}
\BIBentrySTDinterwordspacing

\bibitem{mohammadi2019collaborative}
\BIBentryALTinterwordspacing
J.~Mohammadi and S.~Kolouri, ``Collaborative learning through shared collective
  knowledge and local expertise,'' in \emph{29th International Workshop on
  Machine Learning for Signal Processing}.\hskip 1em plus 0.5em minus
  0.4em\relax IEEE, 2019. [Online]. Available:
  \url{https://doi.org/10.1109/MLSP.2019.8918888}
\BIBentrySTDinterwordspacing

\end{thebibliography}

